Maximum likelihood degree, complete quadrics and ${\mathbb C}^*$-action

We study the maximum likelihood (ML) degree of linear concentration models in algebraic statistics. We relate it to an intersection problem on the variety of complete quadrics. This allows us to provide an explicit, basic, albeit of high computational complexity, formula for the ML-degree. The variety of complete quadrics is an exact analog for symmetric matrices of the permutohedron variety for the diagonal matrices.

==> A2system.tex <==

$$ %%%%% A2 polytope with sections
\begin{xy}<25pt,0pt>:
% central vertex
(0,0)*={\cdot}="z",% (0.2,0)*={0},
% weights
(0,1)*={\circ}="", %(0.2,1)*={\varepsilon_0},
(0.866,0.5)*={\circ}="w1", (1.2,0.5)*={\overline{\omega}_1}, (1.1,0.5)*={},
(0.866,-0.5)*={\circ}="w2", (1.2,-0.5)*={\overline{\omega}_2},% ={x_1},
(0,-1)*={\circ}="e2", %(0.2,-1)*={\varepsilon_2},
(-0.866,-0.5)*={\circ}="", %(-1.1,-0.5)*={\beta_4},
(-0.866,0.5)*={\circ}="", %(-1.1,0.5)*={\varepsilon_3},
% roots
(0.866,1.5)*={\circ}="e1-e2", (1.4,1.3)*={\varepsilon_1-\varepsilon_2},
(1.732,0)*={\circ}="e1-e3", %(2,-0.2)*={},  %(2,0)*={x_1x_2},
(0.866,-1.5)*={\circ}="e2-e3", (1.4,-1.7)*={\varepsilon_2-\varepsilon_3},
(-0.866,-1.5)*={\circ}="e2-e1",% (-1.1,-1.5)*={},
(-1.732,0)*={\circ}="e3-e1", %(-2,0)*={},
(-0.866,1.5)*={\circ}="e3-e2",% (-1.1,1.5)*={},
%z"; "e1-e2" **@{-} *\dir{>}, "z"; "e2-e3" **@{-} *\dir{>},
% 6 x standard
(5.196,3)*={\circ}="S1", (0,-6)*={\circ}="S2", (-5.196,3)*={\circ}="S3",
(5.9,3)*{6\cdot\overline{\omega}_1},
"S1";"S2" **@{.}, "S3";"S2" **@{.}, "S1";"S3" **@{.},
(5.9,-3)*{6\cdot\overline{\omega}_2},
%6 x dual
(5.196,-3)*={\circ}="T1", (0,6)*={\circ}="T2", (-5.196,-3)*={\circ}="T3",
"T1";"T2" **@{.}, "T3";"T2" **@{.}, "T1";"T3" **@{.},
% fixed points exterior
(1.732,3)*={\bullet}="p1",% (1.4,1.3)*={\varepsilon_1-\varepsilon_2},
(3.464,0)*={\bullet}="p2", %(2,-0.2)*={},  %(2,0)*={x_1x_2},
(1.732,-3)*={\bullet}="p3",% (1.4,-1.7)*={\varepsilon_2-\varepsilon_3},
(-1.732,-3)*={\bullet}="p4",% (-1.1,-1.5)*={},
(-3.464,0)*={\bullet}="p5", %(-2,0)*={},
(-1.732,3)*={\bullet}="p6",% (-1.1,1.5)*={},
% fixed points interior
(0,3)*={\bullet}="q1", %(0.2,1)*={\varepsilon_0},
(2.598,1.5)*={\bullet}="q2", (1.2,0.5)*={\overline{\omega}_1}, (1.1,0.5)*={},
(2.598,-1.5)*={\bullet}="q3", (1.2,-0.5)*={\overline{\omega}_2},% ={x_1},
(0,-3)*={\bullet}="q4", %(0.2,-1)*={\varepsilon_2},
(-2.598,-1.5)*={\bullet}="q5", %(-1.1,-0.5)*={\beta_4},
(-2.598,1.5)*={\bullet}="q6", %(-1.1,0.5)*={\varepsilon_3},
% compass at p1
"p1";"q1" **@{=} *\dir{>}, "p1";"q2" **@{=} *\dir{>},
"p1";"p6" **@{-} *\dir{>}, "p1";"p2" **@{-} *\dir{>},
"p1";"e1-e2" **@{-},
"q5";"p5" **@{-} *\dir{>}, "q5";"p4" **@{-} *\dir{>},
"q5";"e2-e1" **@{-} *\dir{>}, "q5";"e3-e1" **@{-} *\dir{>},
"q5";"z" **@{-} *\dir{>},
% edges
%"a5";"a1" **@{-},"b0";"b3" **@{.},
\end{xy}
$$

